Similarity Search for Efficient Active Learning and Search of Rare Concepts

Many active learning and search approaches are intractable for large-scale industrial settings with billions of unlabeled examples. Existing approaches search globally for the optimal examples to label, scaling linearly or even quadratically with the unlabeled data. In this paper, we improve the computational efficiency of active learning and search methods by restricting the candidate pool for labeling to the nearest neighbors of the currently labeled set instead of scanning over all of the unlabeled data. We evaluate several selection strategies in this setting on three large-scale computer vision datasets: ImageNet, OpenImages, and a de-identified and aggregated dataset of 10 billion images provided by a large internet company. Our approach achieved similar mean average precision and recall as the traditional global approach while reducing the computational cost of selection by up to three orders of magnitude, thus enabling web-scale active learning.

==> sections/acknowledgments.tex <==
% From formatting template
\begin{ack}
The Stanford research was supported in part by affiliate members and other supporters of the Stanford DAWN project---Ant Financial, Facebook, Google, Infosys, NEC, and VMware---as well as Toyota Research Institute, Northrop Grumman, Cisco, SAP, and the NSF under CAREER grant CNS-1651570. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of the National Science Foundation. Toyota Research Institute (``TRI'') provided funds to assist the authors with their research but this article solely reflects the opinions and conclusions of its authors and not TRI or any other Toyota entity.
\end{ack}


==> tables/complexity.tex <==
\begin{table}[]
\centering
\caption{Computational complexity for each selection strategy.}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccc}
\toprule
\bfseries Selection Strategy $\phi$ & \bfseries Baseline Complexity ($|\mathcal{P}_r| = |U|$)& \bfseries \flood Complexity ($|\mathcal{P}_r| \leq k|L_r|$) \\
\hline
MaxEnt & $O({|U|})$ & $O(k|L_r|)$  \\
\hline
ID & $O(|U|^2)$  & $O(k^2|L_r|^2)$ \\
\hline
MLP & $O(|U|)$ & $O(k|L_r|)$ \\
\bottomrule
\end{tabular}\label{table:complexity}
}
\end{table}

